Sampling with Barriers: Faster Mixing via Lewis Weights

We analyze Riemannian Hamiltonian Monte Carlo (RHMC) for sampling a polytope defined by $m$ inequalities in $\R^n$ endowed with the metric defined by the Hessian of a convex barrier function. The advantage of RHMC over Euclidean methods such as the ball walk, hit-and-run and the Dikin walk is in its ability to take longer steps. However, in all previous work, the mixing rate has a linear dependence on the number of inequalities. We introduce a hybrid of the Lewis weights barrier and the standard logarithmic barrier and prove that the mixing rate for the corresponding RHMC is bounded by $\tilde O(m^{1/3}n^{4/3})$, improving on the previous best bound of $\tilde O(mn^{2/3})$ (based on the log barrier). This continues the general parallels between optimization and sampling, with the latter typically leading to new tools and more refined analysis. To prove our main results, we have to overcomes several challenges relating to the smoothness of Hamiltonian curves and the self-concordance properties of the barrier. In the process, we give a general framework for the analysis of Markov chains on Riemannian manifolds, derive new smoothness bounds on Hamiltonian curves, a central topic of comparison geometry, and extend self-concordance to the infinity norm, which gives sharper bounds; these properties appear to be of independent interest.

==> intro.tex <==
Sampling in high dimension is a fundamental algorithmic problem~\cite{dyer1991random,lovasz1993random,lovasz2006hit,kannan2012random,lee2018convergence,laddha2020strong,kook2022sampling}. An important and challenging setting is sampling uniformly from a polytope $P = \{x: Ax\ge b\}$. The problem has a rich history and a growing body of applications in very high dimension, approaching a million~\cite{cousins2016practical,haraldsdottir2017chrr,kook2022condition}. While there is a large literature on sampling {\em smooth} densities~\cite{dalalyan2017further,durmus2019analysis,chewi2021analysis,vempala2019rapid,li2022mirror,chewi2022log}, there are relatively few provable methods in constrained, non-smooth settings such as polytope sampling. 
\jon{What is this referring to?  Aren't all of algorithms for sampling from polytops working in the ``constrainted, non-smooth setting?''}

Riemannian Hamiltonian Monte Carlo~\cite{girolami2011riemann} is a Markov chain that follows a random Hamiltonian curve at each step of the chain. More precisely, let the Hamiltonian at a point $x\in \R^n$ for a vector $v \in \R^n$ be defined as 
\begin{align}
    H(x,v)=f(x)+\frac{1}{2} v^{\top}g^{-1}(x) v+\frac{1}{2}\log\det g(x)\label{eq:hmcode}
\end{align}
where $g(x)$ is a positive definite matrix defining a local norm at each point $x$ as $\|u\|_x = \sqrt{u^\top g(x) u}$, and the target density to be sampled is proportional to $e^{-f}$ restricted to the support of $g$. One step of RHMC consists of the following: first pick $v$ from the Gaussian $N(x,g(x)^{-1})$. Then for time $\delta$ follow the Hamiltonian curve jointly on $(x,v)$:
\begin{align}
\frac{dx}{dt} & =\frac{\partial H}{\partial v}(x,v)=g^{-1}(x)v\nonumber \\
\frac{dv}{dt} & =-\frac{\partial H}{\partial x}(x,v)=-\nabla f(x)+\frac{1}{2}\mbox{tr}(g(x)^{-1}Dg(x))-\frac{1}{2} Dg(x)\left[\frac{dx}{dt},\frac{dx}{dt}\right]\label{eq:ham}
\end{align}

The final $x$ at time $\delta$ is the sampled point from the Markov Kernel. A natural choice for the metric $g$ turns out to be the Hessian of a self-concordant barrier function for $P$.
The standard logarithmic barrier, $\phi(x)=-\sum_{i=1}^m \log (a_i^\top x - b_i)$, was used in \cite{lee2018convergence} to prove that the resulting RHMC mixes in $mn^{2/3}$ steps. Improving on this bound is our motivating open problem. 

Using the log barrier implies that the mixing rate has a linear dependence on $m$, the number of inequalities. So we have to look for a ``better" barrier, and what exactly this entails will become clear presently. In this paper, we use a hybrid barrier based on the $p$-Lewis weight barrier $\phi_p$ defined as
\begin{align}
    \phi_p(x) \triangleq \log\det{ \left( \A^\top\W^{1-2/p}\A \right) },\label{eq:lewisbarrier}
\end{align}
where $\W$ is a diagonal matrix whose diagonal entries are the $p$-Lewis weights of the rescaled matrix $\A = S_x^{-1}\A$ and $S_x$ is the diagonal matrix whose entries are the slacks at point $x$, i.e., $(S_x)_{ii} = a_{i}^\top x-b_i$.

\paragraph{History and related work.} Dyer, Frieze and Kannan~\cite{dyer1991random} first showed how to sample a polytope (near-)uniformly in polynomial time. In fact, their algorithm works for sampling a general convex body specified by a membership oracle. Algorithms for sampling are based on Markov chains, and the key parameter is the rate of convergence to the target uniform distribution. The fastest Markov chains for convex bodies have mixing rates that grow at least quadratically in the dimension. These include the ball walk and hit-and-run, and they typically also require additional assumptions on the body (e.g., isotropic position) that need additional time to achieve. Kannan and Narayanan~\cite{kannan2012random} introduced the Dikin walk that exploited the explicit structure of a polytope and gave a mixing time bound of $O(mn)$ from a warm start for a polytope with $m$ facets in $\R^n$. Unlike the ball walk, the steps of the Dikin walk depend on a locally defined ellipsoid. \cite{laddha2020convergence} improved this to $\tilde{O}(n^2)$ by using a weighted Dikin walk. \jon{am I correct that the reference in the previous sentence should be to \cite{laddha2020strong} instead?}
In both papers, the local norm/ellipsoid is defined using the Hessian of a self-concordant convex barrier function. Such functions have played an important role in fast convex optimization~\cite{nesterov1994interior}. In 2017, Lee and Vempala~\cite{lee2017geodesic} used a non-Euclidean process they called the geodesic walk, whose steps follow the solution of an ODE, to reduce the mixing rate to $mn^{3/4}$. In 2018, they improved this to $mn^{2/3}$ using Riemannian Hamiltonian Monte Carlo (RHMC)~\cite{lee2018convergence}.  Advances in self-concordant barriers in the past decade as well as the improvement in the analysis of the Dikin walk suggest that a smaller dependence on $m$, the number of inequalities, which can be much higher than the dimension, should be possible. Nevertheless, improving on the bound of $mn^{2/3}$ has been a major open problem for the past 5 years. Moreover, the new techniques developed as a result of progress on non-Euclidean algorithms suggest that this is a fertile area for further TCS research.

\begin{table}[h]
\centering{}%
\begin{tabular}{|c|l|c|}
\hline 
Year  & Algorithm & Steps\tabularnewline
\hline 
\hline 
1997 \cite{kannan1997random} & Ball walk\textsuperscript{\#} & $n^{3}$ (+$n^5$) \tabularnewline
\hline 
2003 \cite{lovasz2006hit} & Hit-and-run\textsuperscript{\#} & $n^{3}$ (+$n^4$) \tabularnewline
\hline 
2009 \cite{kannan2012random} & Dikin walk & $mn$ \tabularnewline
\hline 
2017 \cite{lee2017geodesic} & Geodesic walk & $mn^{3/4}$ \tabularnewline
\hline
2018 \cite{lee2018convergence} & RHMC with log barrier & $mn^{2/3}$ \tabularnewline
\hline
2020 \cite{laddha2020strong} & Weighted Dikin walk & $n^2$ \tabularnewline
\hline 
2021 \cite{jia2021reducing} & Ball walk\textsuperscript{\#} & $n^2$ (+$n^3$)\tabularnewline
\hline 
\textcolor{red}{This paper} & \textcolor{red}{RHMC with Hybrid barrier} & \textcolor{red}{$m^{1/3}n^{4/3}$} \tabularnewline
\hline 
\end{tabular}\caption{\label{tab:sampling}The complexity of uniformly sampling a polytope from
a warm start. All algorithms have a logarithmic dependence on the warm start parameter and each uses $\widetilde{O}(n)$
bit of randomness. The entries marked \protect\textsuperscript{\#}
are for general convex bodies presented by oracles, while the rest
are for polytopes. The additive terms are pre-processing costs for rounding the polytope.}
\end{table}


==> s-conductance-backup.tex <==
\section{Proof of Theorem~\ref{prop:conductance}}\label{app:sconductance}


Consider a subset $S \subseteq \mathcal S$ with $0.5 \geq \pi(S) = s' \geq s \geq 2\rho$. Then, to show a lower bound for $s$-conductance, we need to lower bound
\begin{align*}
    P(S,S^c)/P(S),
\end{align*}
where $P(.,.) = \int_{x \in S}P_x(S^c)\pi(x)dx$ is the probability that we are in set $S$ and the next step of the Markov chain we escape $S$. Recall that $P_x(.)$ is the Markov kernel, specifiying the distribution of the next step given we are at point $x$. Now assume that the conductance bound does not hold, i.e. there exists such $S$ with 
\begin{align*}
    P(S,S^c)/P(S) = O(\Delta \psi_M).
\end{align*}
Note that because the chain is reversible, we have
\begin{align*}
    P(S,S^c) = P(S^c,S),
\end{align*}
and because $\pi(S) \leq 0.5$, we have
\begin{align}
    P(S^c,S)/P(S^c) \leq P(S,S^c)/P(S) = O(\Delta \psi_M).\label{eq:contradictassumption}
\end{align}
Next, define the set $\tilde S \subseteq S$ to be the points $x$ from which our chance of escaping $S$ is at least $0.01$. Now if $\pi(S) \geq \Delta \psi_{\mathcal M}\pi(S)$, then given that we are in $S$, we have at least $\Delta \psi_{\mathcal M}$ chance of escaping $S$ which contradicts~\eqref{eq:contradictassumption}. This means
\begin{align}
    \pi(\tilde S) \leq \Delta \psi_{\mathcal M} \pi(S).\label{eq:stmp1}
\end{align}
%Similarly, if we define $\tilde S^c \subseteq S^c$ to be the set of points in $S^c$ which has at least $0.01$ chance of escaping to $S$, then
%\begin{align}
%   \pi(\tilde S^c) \leq \Delta \psi_{\mathcal M} \pi(S^c).\label{eq:stmp2}
%\end{align}
On the other hand, note that for point $x_1$ with
%and $x_1 \in S^c - \tilde S^c - {\mathcal M'}^c$ we have $d(x_0, x_1) \leq \Delta$, then from our assumption $TV(P_{x_0}, P_{x_1}) \leq 0.9$ which contradicts the fact that $P_{x_0}$ is concentrated on $S$ and $P_{x_1}$ is concentrated on $S^c$. Therefore, we should have
\begin{align}
    d(S - \tilde S - {\mathcal M'}^c, S^c - \tilde S^c - {\mathcal M'}^c) \geq \Delta.\label{eq:distansebound}
\end{align}
Moreover, from our assumption
\begin{align*}
    p(\mathcal M'^c) \leq \rho \leq \pi(S)/2, \pi(S^c)/2,
\end{align*}
which implies
\begin{align}
    \pi(S - \tilde S - {\mathcal M'}^c) \geq \pi(S) - \pi(\tilde S) - \pi({\mathcal M'}^c)) \geq \pi(S)/2\label{eq:avalii}
\end{align}
and similarly
\begin{align}
    \pi(S^c - \tilde S^c - {\mathcal M'}^c) \geq \pi(S^c)/2.\label{eq:dovomii}
\end{align}
Combining Equations~\eqref{eq:avalii} and~\eqref{eq:dovomii} with Equation~\eqref{eq:distansebound} and using the isoperimetry of $\mathcal M$, we have
\begin{align*}
    \pi(\tilde S \cup \tilde S^c \cup \mathcal M'^c) 
    %\geq \pi(\tilde S \cup \tilde S^c \cup \mathcal M'^c)\Delta\psi_{\mathcal M} 
    = (\pi(S)/2) \times \Delta \psi_{\mathcal M},
\end{align*}


On the other hand, from Equations~\eqref{eq:stmp1} and~\eqref{eq:stmp2} and the fact that $\pi(\mathcal M'^c) \leq \rho \leq \Delta \psi_{\mathcal M}$, 
\begin{align*}
    \pi(\tilde S \cup \tilde S^c \cup \mathcal \psi_{\mathcal M}^c) = O(\Delta )\psi_{\mathcal M},
\end{align*}
which with the correct choice of constants contradicts Equation~\eqref{eq:greaterthan}. This completes the proof.
